Detecting User Exits from Online Behavior: A Duration-Dependent Latent State Model

In order to steer e-commerce users towards making a purchase, marketers rely upon predictions of when users exit without purchasing. Previously, such predictions were based upon hidden Markov models (HMMs) due to their ability of modeling latent shopping phases with different user intents. In this work, we develop a duration-dependent hidden Markov model. In contrast to traditional HMMs, it explicitly models the duration of latent states and thereby allows states to become "sticky". The proposed model is superior to prior HMMs in detecting user exits: out of 100 user exits without purchase, it correctly identifies an additional 18. This helps marketers in better managing the online behavior of e-commerce customers. The reason for the superior performance of our model is the duration dependence, which allows our model to recover latent states that are characterized by a distorted sense of time. We finally provide a theoretical explanation for this, which builds upon the concept of "flow".

==> Covariates_table.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon Nov 18 16:00:24 2019
 Visit depth & 7.68 & 6.76 & 1.00 & 6.00 & 46.00 \\ 
  Time span & 44.79 & 106.45 & 0.00 & 11.00 & 1199.00 \\ 
  Cum. visits on page & 3.77 & 4.25 & 0.00 & 2.00 & 32.00 \\ 
%  Newsletter & 1.44 & 0.63 & 0.00 & 1.72 & 1.72 \\ 
  Weekend & 0.62 & 0.83 & 0.00 & 0.00 & 1.72 \\ 
%  Customer type & 1.55 & 0.52 & 0.00 & 1.72 & 1.72 \\ 
  

==> Demographics_table.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon Nov 18 14:54:07 2019
 Gender & 0.82 & 0.39 & 0.00 & 1.00 & 1.00 \\ 
  Age & 37.95 & 11.84 & 11.00 & 36.00 & 79.00 \\ 
  Age (squared) & 1580.06 & 1008.83 & 121.00 & 1296.00 & 6241.00 \\ 
  

==> Emission_average.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 13 16:38:43 2019 
Goal-directed  & \bfseries 0.2403 & \bfseries 0.2959 & 0.0098 & 0.1280 & 0.0719 & 0.0000 & 0.0904 & 0.0011 & 0.1625 \\ 
  % & [0.0577,0.4163] & [0.0000,0.5604] & [0.0000,0.0958] & [0.0000,0.3807] & [0.0000,0.2126] & [0.0000,0.0000] & [0.0000,0.2223] & [0.0000,0.0065] & [0.0000,0.7060] \\ 

''Sticky`` browsing & 0.0022 & 0.0000 & \bfseries 0.2590 & \bfseries 0.7224 & 0.0152 & 0.0000 & 0.0011 & 0.0000 & 0.0000 \\ 
 %  & [0.0000,0.0094] & [0.0000,0.0000] & [0.1139,0.3742] & [0.5983,0.8671] & [0.0000,0.0502] & [0.0000,0.0000] & [0.0000,0.0072] & [0.0000,0.0000] & [0.0000,0.0000] \\ 
  
''Non-sticky`` browsing & 0.0668 & \bfseries 0.2341 & 0.0000 & 0.0386 & 0.0003 & 0.0000 & 0.0001 & 0.0049 & \bfseries 0.6552 \\ 
 %  & [0.0000,0.1918] & [0.0000,0.9643] & [0.0000,0.0000] & [0.0000,0.1864] & [0.0000,0.0018] & [0.0000,0.0000] & [0.0000,0.0001] & [0.0000,0.0169] & [0.0000,0.9628] \\ 
  

==> Emission_average_hmm.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 20 08:36:09 2019
 Goal-Directed & 0.0627 & 0.0000 & 0.2526 & 0.5736 & 0.0291 & 0.0000 & 0.0218 & 0.0007 & 0.0596 \\ 
  Browsing & 0.0138 & 0.9198 & 0.0000 & 0.0232 & 0.0038 & 0.0000 & 0.0002 & 0.0000 & 0.0393 \\ 
  

==> Emission_covariates.tex <==
% latex table generated in R 3.5.3 by xtable 1.8$-$3 package
% Mon Sep 02 17:05:45 2019
  \textbf{Goal$-$directed} &  &  &  &  &  & \\ 
  Home &   7.75 &   0.34 &   0.32 &   0.32 &     0.39\\ 
   & [ $-$3.52; 22.07] & [$-$13.07; 14.05] & [$-$11.72; 12.99] & [$-$13.07; 13.70] & [$-$12.36; 13.49]\\ 
  Account &  $-$2.45 &   1.06 &   1.02 &   1.04 &      1.08\\ 
   & [$-$17.80; 11.71] & [$-$16.11; 18.18] & [$-$14.41; 16.92] & [$-$15.86; 17.54] & [$-$14.75; 17.61]\\ 
  Overview &   1.78 &   1.30 &   1.28 &   1.31 &   1.20 &\\ 
   & [$-$11.91; 13.61] & [$-$16.12; 18.46] & [$-$14.82; 17.03] & [$-$15.83; 18.14] &  [$-$15.57; 17.12]\\ 
  Product &   4.75 &   0.94 &   0.87 &   0.92 &    0.91 \\ 
   & [ $-$9.93; 18.85] & [$-$13.05; 15.21] & [$-$11.71; 14.10] & [$-$12.59; 15.23] & [$-$12.39; 14.02] \\ 
  Marketing Page &  $-$2.19 &   1.37 &   1.23 &   1.34 &     1.12 \\ 
   & [$-$18.27; 11.60] & [$-$13.87; 17.18] & [$-$12.78; 15.87] & [$-$13.58; 16.73] & [$-$13.08; 16.44] \\ 
  Community &  $-$7.46 &  $-$3.88 &  $-$3.58 &  $-$3.78 &   $-$3.71\\ 
   & [$-$25.84;  9.00] & [$-$25.23; 16.70] & [$-$23.10; 15.30] & [$-$24.77; 16.33] &  [$-$24.23; 15.47] \\ 
  Checkout &   4.45 &   2.03 &   1.89 &   1.98 &   2.03 \\ 
   & [ $-$6.50; 18.48] & [ $-$8.89; 13.58] & [ $-$8.20; 12.20] & [ $-$8.75; 13.18] & [ $-$8.36; 12.63] \\ 
  Order &  $-$3.97 &  $-$0.92 &  $-$0.90 &  $-$0.92 & $-$0.89 \\ 
   & [$-$24.73; 14.09] & [$-$22.30; 19.71] & [$-$20.71; 17.62] & [$-$22.40; 18.85] & [$-$21.47; 18.03]  \\ 
  Exit &  $-$4.39 &  $-$2.20 &  $-$2.02 &  $-$2.14 &  $-$2.08  \\ 
   & [$-$24.36; 14.58] & [$-$23.24; 17.03] & [$-$21.19; 15.49] & [$-$22.80; 16.46] & [$-$21.70; 16.06]  \\ 
  \textbf{``Sticky'' browsing} &  &  &  &  &  &   \\ 
  Home &   2.65 &   1.07 &   1.07 &   1.05 &   1.21  \\ 
   & [$-$14.22; 18.03] & [$-$15.69; 16.75] & [$-$14.05; 15.60] & [$-$15.46; 16.49] & [$-$14.55; 15.82] \\ 
  Account &   3.80 &  $-$1.75 &  $-$1.62 &  $-$1.72 &   $-$1.58 \\ 
   & [$-$17.55; 23.10] & [$-$26.12; 19.39] & [$-$23.54; 17.78] & [$-$25.29; 18.99] & [$-$24.31; 18.56] \\ 
  Overview &   1.89 &   4.46 &   4.10 &   4.36 &    4.13  \\ 
   & [$-$12.86; 16.55] & [ $-$8.34; 18.84] & [ $-$7.34; 17.55] & [ $-$7.84; 18.84] & [ $-$7.76; 17.73]  \\ 
  Product &   9.04 &   3.43 &   3.21 &   3.37 &   3.20  \\ 
   & [ $-$2.35; 21.39] & [ $-$8.57; 15.69] & [ $-$7.77; 14.49] & [ $-$8.35; 15.56] & [ $-$7.92; 14.78] \\ 
  Marketing Page &   6.95 &   1.06 &   0.90 &   1.00 &   1.03 \\ 
   & [ $-$5.19; 18.56] & [$-$12.28; 14.76] & [$-$11.52; 13.39] & [$-$12.30; 14.45] & [$-$11.53; 13.60]  \\ 
  Community &  $-$5.33 &  $-$2.92 &  $-$2.69 &  $-$2.85 &  $-$2.79  \\ 
   & [$-$22.88; 10.18] & [$-$23.77; 16.97] & [$-$21.83; 15.36] & [$-$23.67; 16.23] & [$-$22.57; 15.84]  \\ 
  Checkout &  $-$3.35 &   1.78 &   1.63 &   1.73 &    1.69  \\ 
   & [$-$20.44; 13.69] & [$-$16.21; 19.13] & [$-$14.94; 17.47] & [$-$15.60; 19.06] &  [$-$15.30; 17.89]  \\ 
  Order &  $-$4.51 &  $-$3.27 &  $-$3.03 &  $-$3.19 &  $-$3.14  \\ 
   & [$-$24.77; 14.70] & [$-$24.86; 18.21] & [$-$22.81; 16.40] & [$-$24.22; 18.01] & [$-$23.47; 17.07]  \\ 
  Exit &  $-$7.56 &  $-$3.29 &  $-$3.04 &  $-$3.20 &   $-$3.18  \\ 
   & [$-$26.27;  9.22] & [$-$24.86; 17.51] & [$-$22.68; 16.08] & [$-$24.46; 17.12] & [$-$23.18; 16.70] \\ 
  \textbf{``Non$-$sticky'' browsing} &  &  &  &    &  \\ 
  Home &  15.46 &  $-$2.37 &  $-$2.16 &  $-$2.31  &  $-$2.25  \\ 
   & [ $-$3.59; 34.56] & [$-$30.42; 17.00] & [$-$28.28; 15.70] & [$-$29.96; 16.42] & [$-$29.71; 15.77]  \\ 
  Account &  $-$0.51 &  $-$2.00 &  $-$1.78 &  $-$1.94 &   $-$1.83 \\ 
   & [$-$23.45; 21.61] & [$-$23.45; 17.34] & [$-$21.44; 15.96] & [$-$22.96; 17.10] & [$-$22.15; 16.46]  \\ 
  Overview &  $-$1.84 &  $-$0.84 &  $-$0.84 &  $-$0.83 &   $-$0.92 \\ 
   & [$-$20.00; 16.15] & [$-$22.76; 20.87] & [$-$20.91; 18.86] & [$-$22.56; 20.34] &  [$-$21.34; 19.44]  \\ 
  Product &   3.96 &  $-$0.42 &  $-$0.42 &  $-$0.42 &   $-$0.43\\ 
   & [$-$16.27; 24.96] & [$-$21.82; 19.17] & [$-$20.02; 17.45] & [$-$21.52; 18.53] &  [$-$20.74; 17.91] \\ 
  Marketing Page &  $-$4.36 &   0.10 &  $-$0.05 &   0.06 &  $-$0.04 \\ 
   & [$-$23.96; 13.88] & [$-$21.93; 21.13] & [$-$19.85; 19.43] & [$-$21.42; 20.75] & [$-$20.67; 19.87]  \\ 
  Community &  $-$5.65 &  $-$3.02 &  $-$2.79 &  $-$2.94 & $-$2.89 \\ 
   & [$-$24.49; 11.85] & [$-$24.59; 18.17] & [$-$22.60; 16.49] & [$-$23.94; 17.90] &  [$-$23.36; 17.04]  \\ 
  Checkout &  $-$3.44 &   0.41 &   0.43 &   0.42 &  0.37\\ 
   & [$-$23.08; 14.76] & [$-$21.76; 23.00] & [$-$19.87; 20.80] & [$-$21.63; 22.13] & [$-$20.89; 21.11]  \\ 
  Order &  $-$3.53 &   4.53 &   4.23 &   4.43 &  4.42 \\ 
   & [$-$22.05; 17.11] & [$-$17.96; 28.02] & [$-$16.09; 26.21] & [$-$17.22; 27.76] & [$-$16.55; 27.04] \\ 
  Exit &   2.34 &   3.32 &   3.08 &   3.23 &  3.33 \\ 
   & [$-$17.28; 18.27] & [$-$16.53; 25.86] & [$-$15.21; 23.79] & [$-$16.20; 25.03] &  [$-$15.52; 24.95] \\ 
  

==> Emission_covariates_V2.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Fri Aug 30 14:55:17 2019
 State 1 &  &  &  &  &  \\ 
   & View &  & 7.75 & -2.46 & 0.32 \\ 
   &  &  & [-2.47,20.71] & [-24.79,11.08] & [-7.93,8.96] \\ 
   & Buy &  & -2.45 & 1.05 & -0.25 \\ 
   &  &  & [-16.79,9.93] & [-11.59,13.25] & [-13.47,11.84] \\ 
   & Exit &  & 1.78 & -0.20 & -0.54 \\ 
   &  &  & [-10.16,12.32] & [-12.02,10.15] & [-9.80,10.47] \\ 
  State 2 &  &  &  &  &  \\ 
   & View &  & 4.75 & 2.66 & 0.03 \\ 
   &  &  & [-7.97,16.54] & [-12.32,14.00] & [-11.17,12.37] \\ 
   & Buy &  & -2.19 & 0.22 & 0.72 \\ 
   &  &  & [-16.93,9.54] & [-12.23,12.29] & [-12.21,13.12] \\ 
   & Exit &  & -7.46 & -5.10 & -4.51 \\ 
   &  &  & [-24.08,6.97] & [-24.62,13.69] & [-22.51,12.90] \\ 
  State 3 &  &  &  &  &  \\ 
   & View &  & 4.45 & 3.06 & 3.33 \\ 
   &  &  & [-5.38,14.54] & [-7.42,13.55] & [-4.67,12.19] \\ 
   & Buy &  & -3.97 & 4.98 & 3.65 \\ 
   &  &  & [-23.48,11.01] & [-13.40,20.67] & [-11.27,18.00] \\ 
   & Exit &  & -4.39 & 0.54 & -1.78 \\ 
   &  &  & [-21.53,13.04] & [-21.36,18.19] & [-19.22,13.39] \\ 
  

==> Emission_intercept.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Tue Jun 04 16:57:28 2019
 Prob(View) &  &  &  \\ 
   & State 1 & 0.531 & [0.002,1.000] \\ 
   & State 2 & \bfseries{0.987} & [0.973,1.000] \\ 
   & State 3 & 0.576 & [0.064,1.000] \\ 
  Prob(Buy) &  &  &  \\ 
   & State 1 & \bfseries{0.039} & [0.000,0.080] \\ 
   & State 2 & 0.001 & [0.000,0.005] \\ 
   & State 3 & 0.018 & [0.000,0.033] \\ 
  Prob(Exit) &  &  &  \\ 
   & State 1 & \bfseries{0.431} & [0.000,0.965] \\ 
   & State 2 & 0.011 & [0.000,0.022] \\ 
   & State 3 & 0.406 & [0.000,0.915] \\ 
  

==> Summary_statistics.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Tue Jun 04 17:31:01 2019
 View & 3.35 & 5.49 & 0.00 & 44.00 \\ 
  Buy & 0.17 & 0.95 & 0.00 & 9.00 \\ 
  Exit & 0.95 & 0.22 & 0.00 & 1.00 \\ 
  Session length (in clicks) & 4.63 & 6.16 & 1.00 & 44.00 \\ 
  Session length (in mins) & 7.33 & 14.46 & 0.00 & 126.65 \\ 
  

==> Summary_statistics_digi.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 20 09:31:36 2019
  Visit depth (in pages) & 9.80 & 6.33 & 9.71 & 5.74 & 10.09 & 7.80 \\ 
  Session duration (in min) & 6.04 & 9.31 & 2.16 & 2.37 & 17.10 & 12.36 \\ 
	\midrule
	Page categories$^a$ \\
  \quad \textsc{Home} & 1.13 & 1.20 & 1.21 & 1.21 & 0.90 & 1.12 \\ 
  \quad \textsc{Account} & 0.85 & 1.93 & 0.89 & 1.97 & 0.73 & 1.81 \\ 
  \quad \textsc{Overview} & 1.99 & 3.02 & 1.81 & 2.70 & 2.52 & 3.74 \\ 
  \quad \textsc{Product} & 3.92 & 4.45 & 3.61 & 4.33 & 4.82 & 4.70 \\ 
  \quad \textsc{Marketing Page} & 0.85 & 1.62 & 1.00 & 1.78 & 0.43 & 0.95 \\ 
  \quad \textsc{Community} & 0.00 & 0.07 & 0.01 & 0.08 & 0.00 & 0.00 \\ 
  \quad \textsc{Checkout} & 0.25 & 0.71 & 0.18 & 0.61 & 0.43 & 0.91 \\ 
  

==> Summary_statistics_segmented.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Tue Jun 04 19:34:54 2019
 Across sessions with exit &  &  &  &  &  \\ 
   & View & 3.07 & 5.28 & 0.00 & 44.00 \\ 
   & Session length (in clicks) & 4.06 & 5.24 & 1.00 & 44.00 \\ 
   & Session length (in mins) & 7.33 & 14.46 & 0.00 & 126.65 \\ 
  Across sessions with purchase &  &  &  &  &  \\ 
   & View & 8.60 & 7.00 & 2.00 & 24.00 \\ 
   & Session length (in clicks) & 15.40 & 11.32 & 4.00 & 34.00 \\ 
   & Session length (in mins) & 19.79 & 20.34 & 4.48 & 65.10 \\ 
  

==> duration_parameters.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Fri Aug 30 14:01:59 2019
Goal-directed & 0.44 & 0.95 & 2.39 \\ 
   & [0.24; 0.84] & [0.77; 1.12] &  \\ 
  ''Sticky`` browsing & 0.16 & 1.02 & 5.98 \\ 
   & [0.10; 0.22] & [0.89; 1.20] &  \\ 
  ''Non-sticky`` browsing & 0.76 & 1.36 & 1.26 \\ 
   & [0.18; 1.00] & [1.01; 1.86] &  \\ 
  

==> duration_parameters_hmm.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 20 15:56:55 2019
 Goal-directed & 0.02 & 40.24 \\ 
   & [0.02,0.03] &  \\ 
  Browsing & 0.24 & 4.11 \\ 
   & [0.20,0.29] &  \\ 
  

==> initial.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Fri Aug 30 14:49:52 2019
 Goal-directed search & 0.24 & [0.07; 0.56] \\ 
  ''Sticky`` browsing & \bfseries{0.40} & [0.27; 0.64] \\ 
  ''Non-sticky`` browsing & 0.37 & [0.03; 0.59] \\ 
  

==> initial_hmm.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 20 08:53:37 2019
 Goal-directed & 0.48 & [0.44,0.50] \\ 
  Browsing & \bfseries{0.52} & [0.50,0.56] \\ 
  

==> model_selection.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon Jun 10 12:35:57 2019
 1 & 810.24 \\ 
  2 & 792.24 \\ 
  3 & \textbf{743.02} \\ 
  4 & 747.74 \\ 
  

==> model_selection_and_performance.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Sun Jun 16 09:45:56 2019
 1 & 9328.7 & 9312.0 & 0.6745 & 0.1268 \\ 
  2 & 9232.1 & 9207.8 & 0.6312 & 0.0897 \\ 
  3 & \bfseries 8735.6& \bfseries 8785.9 & \bfseries 0.7176 & \bfseries 0.1364 \\ 
  4 & 8395.7& 8475.4 & 0.6112 & 0.1214 \\ 
  

==> model_selection_and_performance_hmm.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Sun Jun 16 09:51:04 2019
 1 & 9719.4 & 9311.7 & 0.6751 & 0.1270 \\ 
  2 & \bfseries 8312.7 & \bfseries 8306.8 &\bfseries 0.6411 & \bfseries 0.1221 \\ 
  3 & 7892.1 & 7873.1 & 0.6394 & 0.1242 \\ 
4 & 7603.2 & 7568.4 & 0.5397 &0.0753 \\ 
5 & 7497.7 & 7484.0 & 0.5371 &0.0949 \\ 

==> model_selection_hmm.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Sun Jun 16 09:49:04 2019
 1 & 811.282 & 0.743 & 0.373 \\ 
  2 & \textbf{723.602} & \textbf{0.764} & \textbf{0.437} \\ 
  3 & 726.805 & 0.770 & 0.447 \\ 
  4 & 720.497 & 0.759 & 0.422 \\ 
  

==> performance_comparison.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Jun 05 18:38:06 2019
 2-State HMM & 0.76 & 0.44 & 0.81 \\ 
  3-State HSMM & \textbf{0.78} & \textbf{0.45} & \textbf{0.91} \\ 
  

==> plot_trans_prob.tex <==
% Created by tikzDevice version 0.12 on 2019-09-03 16:21:24
% !TEX encoding = UTF-8 Unicode


==> transition_covariates.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 13 17:00:39 2019
 1 & -0.36 & -0.19 & 0.37 \\ 
   & [-10.18,9.00] & [-6.88,6.05] & [-6.25,6.93] \\ 
  2 & 0.19 & 0.10 & 0.15 \\ 
   & [-7.25,6.88] & [-9.59,9.54] & [-7.15,6.99] \\ 
  3 & 0.36 & -0.76 & 0.06 \\ 
   & [-6.94,7.66] & [-8.97,6.15] & [-10.59,9.79] \\ 
  

==> transition_intercept.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Wed Nov 13 17:00:25 2019
 1 & 0.45 & 0.35 & 0.20 \\ 
   & [0.00,1.00] & [0.00,0.93] & [0.00,0.63] \\ 
  2 & 0.23 & 0.44 & 0.33 \\ 
   & [0.00,0.97] & [0.00,1.00] & [0.00,0.88] \\ 
  3 & 0.22 & 0.34 & 0.44 \\ 
   & [0.00,0.84] & [0.00,0.98] & [0.00,1.00] \\ 
  
